A Computational Design and Evaluation Tool for 3D Structures with Planar Surfaces

Three dimensional (3D) structures composed of planar surfaces can be build out of accessible materials using easier fabrication technique with shorter fabrication time. To better design 3D structures with planar surfaces, realistic models are required to understand and evaluate mechanical behaviors. Existing design tools are either effort-consuming (e.g. finite element analysis) or bounded by assumptions (e.g. numerical solutions). In this project, We have built a computational design tool that is (1) capable of rapidly and inexpensively evaluating planar surfaces in 3D structures, with sufficient computational efficiency and accuracy; (2) applicable to complex boundary conditions and loading conditions, both isotropic materials and orthotropic materials; and (3) suitable for rapid accommodation when design parameters need to be adjusted. We demonstrate the efficiency and necessity of this design tool by evaluating a glass table as well as a wood bookcase, and iteratively designing an origami gripper to satisfy performance requirements. This design tool gives non-expert users as well as engineers a simple and effective modus operandi in structural design.

==> Packages.tex <==
% packages


\usepackage{hyperref}

\usepackage[left=1.25in, right=1.25in, top=1in, bottom=1in]{geometry}

\usepackage{setspace}
% \onehalfspacing

\usepackage{subfiles}

\usepackage{caption}
% \usepackage{subcaption}
\usepackage{graphics} % for pdf, bitmapped graphics files


\usepackage{epsfig} % for postscript graphics files
\usepackage{epstopdf}
\usepackage{mathptmx} % assumes new font selection scheme installed
\usepackage{times} % assumes new font selection scheme installed
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed
\usepackage{mathtools}
% \usepackage{cite}
\usepackage{float} % float the table when using [H]
% \usepackage[final]{pdfpages}

\usepackage{color} % color the text

\usepackage[utf8]{inputenc}

\usepackage{comment} % for commenting

\usepackage{subcaption}

\usepackage{siunitx} % for SI units
\let\DeclareUSUnit\DeclareSIUnit
\let\US\SI
\DeclareUSUnit\inch{"}

\makeatletter\newcommand*{\at}{@}\makeatother

\renewcommand{\bottomfraction}{0.85}

\usepackage{textcomp}  % for copyright
\usepackage[export]{adjustbox}  % adjust figure alignment

\usepackage{array}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\usepackage{multirow}

\usepackage{setspace}  % change line spacing inside document

\usepackage{esvect}

\usepackage{url}

\usepackage{amsbsy}

\usepackage{array}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\usepackage{multirow}

\usepackage{mathtools}
\usepackage{bm}
\usepackage{esvect}

\usepackage{tablefootnote}

\usepackage{hyperref}
